Findings of the 2023 ML-SUPERB Challenge: Pre-Training and Evaluation over More Languages and Beyond

The 2023 Multilingual Speech Universal Performance Benchmark (ML-SUPERB) Challenge expands upon the acclaimed SUPERB framework, emphasizing self-supervised models in multilingual speech recognition and language identification. The challenge comprises a research track focused on applying ML-SUPERB to specific multilingual subjects, a Challenge Track for model submissions, and a New Language Track where language resource researchers can contribute and evaluate their low-resource language data in the context of the latest progress in multilingual speech recognition. The challenge garnered 12 model submissions and 54 language corpora, resulting in a comprehensive benchmark encompassing 154 languages. The findings indicate that merely scaling models is not the definitive solution for multilingual speech tasks, and a variety of speech/voice types present significant challenges in multilingual speech processing.

==> tables/1h-hidden-set.tex <==
\resizebox {0.75\linewidth} {!} {
\begin{tabular}{l|c|c|c|cc|c}
\toprule
\multirow{2}{*}{SSL} & Monolingual ASR & Multilingual ASR & LID & \multicolumn{2}{c|}{Multilingual ASR + LID} & \multirow{3}{*}{SUPERB$_{s}$} \\
& CER/PER & CER & ACC & ACC & CER &   \\
\midrule
FBANK & 70.7 & 68.4 & 14.7 & 37.1 & 65.8 & 0 \\
\rowcolor{mono} wav2vec2-base \cite{baevski2020wav2vec} & 54.2 & 47.0 & 60.2 & 42.2 & 42.6 & 620.3 \\
\rowcolor{regional} wav2vec2-base-23 \cite{wang2021voxpopuli} & 56.1 & 49.9 & 57.0 & 59.9 & 48.5 & 654.2 \\
\rowcolor{multi} XLSR-128 \cite{babu2021xls} & 49.2 & 39.0 & \textbf{70.2} & \textbf{70.7} & \textbf{37.7} & 962.0 \\
\rowcolor{mono} HuBERT-base \cite{hsu2021hubert} & 53.8 & 47.2 & 65.1 & 63.1 & 45.8 & 760.5 \\
\rowcolor{mono} HuBERT-large \cite{hsu2021hubert} & 52.3 & 47.3 & 57.9 & 58.9 & 45.0 & 730.9\\
\rowcolor{regional} mHuBERT-base \cite{lee2022textless} & 53.3 & 46.1 & 65.3 & 61.6 & 45.5 & 771.2 \\
\midrule
\rowcolor{multi} MMS-300m & 51.0 & 42.2 & 45.3 & 66.2 & 40.8 & 774.7 \\
\rowcolor{multi} MMS-1b & \textbf{46.8} & \textbf{37.4} & 65.4 & 60.9 & 39.5 & 933.9 \\
\midrule
\rowcolor{multi} CV-HuBERT-base & 52.3 & 43.7 & 68.9 & 68.9 & 42.6 & 857.3 \\
\rowcolor{multi} CV-HuBERT-base (40ms) & 63.2 & 52.0 & 66.0 & 57.4 & 59.0 & 547.6 \\
\rowcolor{multi} CV-HuBERT-base (80ms) & 67.9 & 69.8 & 50.9 & 40.5 & 69.1 & 179.0\\
\rowcolor{multi} CV-HuBERT-MR-base & 54.8 & 44.5 & 66.7 & 66.7 & 43.0 & 804.8 \\
\midrule
\rowcolor{multi} EFFUSE (W2V2+XLSR) & 50.6 & 41.9 & 57.3 & 63.7 & 40.6 & 826.9\\
\rowcolor{multi} EFFUSE (HuBERT+XLSR) & 49.1 & 40.3 & 55.9 & 66.4 & 39.3 & 865.0\\
\midrule
\rowcolor{multi} NWHC1 & 47.7 & 38.9 & 69.4 & 69.4 & 38.5 & \textbf{966.5} \\
\rowcolor{multi} NWHC2 & 47.8 & 38.9 & 68.9 & 68.9 & 38.4 & 961.8\\
\midrule
\rowcolor{multi} WavLabLM-base & 47.2 & 47.6 & 58.2 & 58.1 & 46.8 & 772.1\\
\rowcolor{multi} WavLabLM-large-EK & 50.3 & 54.2 & 55.7 &  45.4 & 60.3 & 567.9 \\
\rowcolor{multi} WavLabLM-large-MK & 50.3 & 55.6 & 62.0 & 61.0 & 53.7 & 672.4\\
\rowcolor{multi} WavLabLM-large-MS & 50.7 & 55.5 & 61.6 & 59.2 & 53.9 & 659.7 \\

\bottomrule
\end{tabular}
}

==> tables/1h-public-set.tex <==
\resizebox {0.8\linewidth} {!} {
\begin{tabular}{l|c|cc|c|ccc|c}
\toprule
\multirow{3}{*}{SSL} & Monolingual ASR & \multicolumn{2}{c|}{Multilingual ASR} & \multicolumn{1}{c|}{LID} & \multicolumn{3}{c|}{Multilingual ASR + LID} & \multirow{3}{*}{SUPERB$_{s}$} \\
&          &             Normal & Few-shot & Normal & \multicolumn{2}{c}{Normal} & \multicolumn{1}{c|}{Few-shot} \\
& CER/PER & CER & CER & ACC & ACC & CER & \multicolumn{1}{c|}{CER} &  \\
\midrule
FBANK & 63.7 & 59.3 & 57.4 & 9.3  & 43.5 & 58.6 & 58.1 & 0 \\
\rowcolor{mono} wav2vec2-base \cite{baevski2020wav2vec}& 35.9 & 35.5 & 44.3 & 80.8& 83.6  & 32.1 & 42.6 & 707.8 \\
\rowcolor{regional} wav2vec2-base-23 \cite{wang2021voxpopuli} & 35.1 & 32.0 & 42.2 & 71.9 & 66.3 & 30.9 & 43.0 & 676.5 \\
\rowcolor{multi} XLSR-128 \cite{babu2021xls} & 30.6 & 22.0 & 39.3 & 87.9 & 85.6  & 22.9 & 42.4 & 854.2\\
\rowcolor{mono} HuBERT-base \cite{hsu2021hubert} & 35.3 & 31.4 & 42.7 & 86.1 & 86.0 & 30.9 & 41.8 & 757.0 \\
\rowcolor{mono} HuBERT-large \cite{hsu2021hubert} & 32.2 & 37.7 & 43.5 & 64.1 & 77.7 & 35.1 & 42.2 & 659.8  
 \\
\rowcolor{regional} mHuBERT-base \cite{lee2022textless} & 33.0 & 33.4 & 43.6 & 72.5 & 70.9 & 29.7 & 43.1 &  
692.1 \\
\midrule
\rowcolor{multi} MMS-300m & 30.5 & 24.0 & 36.5 & 84.3 & 74.3 & 30.0 & 29.2 & 841.3 \\
\rowcolor{multi} MMS-1b & \textbf{25.7} & \textbf{18.1} & \textbf{30.8} & 86.1 & 74.8 & 25.5 & \textbf{24.8} & \textbf{943.2} \\
\midrule
\rowcolor{multi} CV-HuBERT-base & 32.9 & 27.5 & 40.8 & 84.0 & 87.3 & 28.2 & 41.1 & 796.7\\
\rowcolor{multi} CV-HuBERT-base (40ms) & 62.6 & 52.0 & 53.0 & 83.0 & 83.3 & 52.3 & 53.4 & 380.4 \\
\rowcolor{multi} CV-HuBERT-base (80ms) & 67.6 & 70.7 &  64.1 & 57.2 & 39.4 & 70.4 & 64.4 & 16.2\\
\rowcolor{multi} CV-HuBERT-MR-base & 38.3  & 28.3 & 40.8 & 86.0 & 84.5 & 30.6 & 41.0 & 755.0\\
\midrule
\rowcolor{multi} EFFUSE (W2V2+XLSR) & 28.9 & 24.4 & 40.2 & 13.5 & 87.8 & 24.4 & 39.3  & 624.6 \\
\rowcolor{multi} EFFUSE (HuBERT+XLSR) & 29.5 & 23.5 & 38.3 &   79.0 & 89.9 & 23.3 & 37.6 & 849.8\\
\midrule
\rowcolor{multi} NWHC1 & 30.5 & 21.5 & 38.6 & 87.4 & \textbf{90.6} & \textbf{21.5} & 38.2 & 878.6 \\
\rowcolor{multi} NWHC2 & 30.5 & 21.6 & 39.3 & \textbf{88.1} & \textbf{90.6} & 21.8 & 38.8 & 875.3 \\
\midrule
\rowcolor{multi} WavLabLM-base & 37.6 &  39.6 & 44.5 & 56.5 & 67.8 & 38.2 & 43.9 & 561.8\\
\rowcolor{multi} WavLabLM-large-EK &  33.7 & 33.5 & 41.9 & 83.4 & 79.9 & 33.1 & 41.3 & 741.7\\
\rowcolor{multi} WavLabLM-large-MK & 32.3 & 32.8 & 42.8 & 79.0 & 79.6 & 32.8 & 42.4 & 732.7 \\
\rowcolor{multi} WavLabLM-large-MS & 32.8 & 31.9 & 42.8& 81.1 & 80.0 & 32.2 & 41.2  & 743.3\\
\bottomrule
\end{tabular}
}

